Heterogeneous Verification of an Autonomous Curiosity Rover

The Curiosity rover is one of the most complex systems successfully deployed in a planetary exploration mission to date. It was sent by NASA to explore the surface of Mars and to identify potential signs of life. Even though it has limited autonomy on-board, most of its decisions are made by the ground control team. This hinders the speed at which the Curiosity reacts to its environment, due to the communication delays between Earth and Mars. Depending on the orbital position of both planets, it can take 4--24 minutes for a message to be transmitted between Earth and Mars. If the Curiosity were controlled autonomously, it would be able to perform its activities much faster and more flexibly. However, one of the major barriers to increased use of autonomy in such scenarios is the lack of assurances that the autonomous behaviour will work as expected. In this paper, we use a Robot Operating System (ROS) model of the Curiosity that is simulated in Gazebo and add an autonomous agent that is responsible for high-level decision-making. Then, we use a mixture of formal and non-formal techniques to verify the distinct system components (ROS nodes). This use of heterogeneous verification techniques is essential to provide guarantees about the nodes at different abstraction levels, and allows us to bring together relevant verification evidence to provide overall assurance.

==> dia/fullspec.tex <==
\hspace{-10pt}
\scalebox{0.49}{
\begin{tikzpicture}[node distance=2em]
\node (agent) [process] {\parbox[t][][t]{3cm}{\centering Agent}};
\node(agentspec)[left of = agent, xshift = -20em, yshift= -2em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_A}$:} $\overline{o_R} \land$ $n \in \mathbb{N} \land Wayp = \langle w_1, \ldots, w_n \rangle \land W = Wayp$ \\ 
		\textbf{$\overline{o_A}$:} act\\
		$\mathcal{A}_A(\overline{i_A}): \mathcal{G}_R(\overline{o_R})$\\
		$\mathcal{G}_A(\overline{o_A}):  W = Wayp\iff W = {\emptyset}$\\
		$\t2 \land start \Rightarrow act = patrol(w_1) \land w_1 \notin W $ \\ %when it receives start from rosbridge it sends the message to patrol the first waypoint
		\t2 $\land move\_result = \top \Rightarrow $\\ 
		\t3 $act = patrol(w_1) \land w_1 \notin W $ %when it receives a success move result message, then it sends the message to patrol the next waypoint
		\end{tabular}}};

\node (rosbridge) [process, below of = agent, yshift = -4em] {\parbox[t][][t]{3cm}{\centering Rosbridge}};
\node(rosbridgespec)[right of = rosbridge, xshift = 9em, yshift = 3em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_R}$:} $\overline{o_A} \land \overline{o_{As}} \land \overline{o_{Ms}} \land \overline{o_{Ws}}$\\ 
		\textbf{$\overline{o_R}$:} msg\\
		$\mathcal{A}_R(\overline{i_R}): \mathcal{G}_A(\overline{o_A}) \land \mathcal{G}_{As}(\overline{o_{As}}) \land \mathcal{G}_{Ms}(\overline{o_{Ms}}) \land \mathcal{G}_{Ws}(\overline{o_{Ws}})$\\
		$\mathcal{G}_R(\overline{o_R}): msg = act \lor msg = \overline{o_{As}} \lor msg = \overline{o_{Ms}} \lor msg = \overline{o_{Ws}} $ %this node only receives and sends messages, and ideally we would want to guarantee that the message is not modified $ %this node only receives and sends messages, and ideally we would want to guarantee that the message is not modified
		\end{tabular}}};

\node (armclient) [process, below of = rosbridge, yshift = -4em, xshift = -17em] {\parbox[t][][t]{3cm}{\centering Arm Client}};
\node(armclientspec)[left of = armclient, yshift = 2.5em, xshift = -10em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Ac}}$:} $\overline{o_R} \land \overline{o_{As}}$\\ 
		\textbf{$\overline{o_{Ac}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Ac}(\overline{i_{Ac}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{As}(\overline{o_{As}})$\\
		$\mathcal{G}_{Ac}(\overline{o_{Ac}}): g = act $ %
		\end{tabular}}};

\node (mastclient) [process, below of = rosbridge, yshift = -4em, xshift = 4em] {\parbox[t][][t]{3cm}{\centering Mast Client}};
\node(mastclientspec)[left of = mastclient, xshift = -9.5em, yshift = -2em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Mc}}$:} $\overline{o_R} \land \overline{o_{Ms}}$\\ 
		\textbf{$\overline{o_{Mc}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Mc}(\overline{i_{Mc}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{Ms}(\overline{o_{Ms}})$\\
		$\mathcal{G}_{Mc}(\overline{o_{Mc}}): g = act$ %
		\end{tabular}}};


\node (wheelsclient) [process, below of = rosbridge, yshift = -4em, xshift = 16em] {\parbox[t][][t]{3cm}{\centering Wheels Client}};
\node(wheelsclientspec)[ right of = wheelsclient, xshift = 6em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Wc}}$:} $\overline{o_R} \land \overline{o_{Ws}}$\\ 
		\textbf{$\overline{o_{Wc}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Wc}(\overline{i_{Wc}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{Ws}(\overline{o_{Ws}})$\\
		$\mathcal{G}_{Wc}(\overline{o_{Wc}}): g=act $ %
		\end{tabular}}};

\node (armserver) [process, below of = armclient, yshift = -6em] {\parbox[t][][t]{3cm}{\centering Arm Server}};
\node(armserverspec)[below of = armserver, yshift = -2.5em, xshift = -5em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{As}}$:} $\overline{o_{Ac}}$\\ 
		\textbf{$\overline{o_{As}}$: $r\in\{\top , \bot \}$} \\
		$\mathcal{A}_{As}(\overline{i_{As}}): \mathcal{G}_{Ac}(\overline{o_{Ac}})$\\
		$\mathcal{G}_{As}(\overline{o_{As}}): r = \top \Rightarrow executed(g)$ %
		\end{tabular}}};

\node (mastserver) [process, below of = mastclient, yshift = -6em] {\parbox[t][][t]{3cm}{\centering Mast Server}};
\node(mastserverspec)[left of = mastserver, xshift = -10em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Ms}}$:} $\overline{o_{Mc}}$\\ 
		\textbf{$\overline{o_{Ms}}$:$r\in \{\top , \bot\}$} \\
		$\mathcal{A}_{Ms}(\overline{i_{Ms}}): \mathcal{G}_{Mc}(\overline{o_{Mc}})$\\
		$\mathcal{G}_{Ms}(\overline{o_{Ms}}): r = \top \Rightarrow executed(g) $ %
		\end{tabular}}};

\node (wheelsserver) [process, below of = wheelsclient, yshift = -6em] {\parbox[t][][t]{3cm}{\centering Wheels Server}};
\node(wheelsserverspec)[below of = wheelsserver, xshift = 6em, yshift = -3em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Ws}}$:} $\overline{o_{Wc}}$\\ 
		\textbf{$\overline{o_{Ws}}$: $r \in \{\top , \bot\}$} \\
		$\mathcal{A}_{Ws}(\overline{i_{Ws}}): \mathcal{G}_{Wc}(\overline{o_{Wc}})$\\
		$\mathcal{G}_{Ws}(\overline{o_{Ws}}): r = \top \Rightarrow executed(g) $ %
		\end{tabular}}};

\node (robotstate) [process, below of = mastserver, yshift = -8em] {\parbox[t][][t]{3cm}{\centering Robot State Publisher}};
%\node(robotstatespec)[right of = robotstate, yshift = -1em, xshift = 9em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
%		\textbf{$\overline{i_{Rsp}}$:} $\overline{o_{As}} \land \overline{o_{Ms}} \land \overline{o_{Ws}}$\\ 
%		\textbf{$\overline{o_{Rsp}}$:} \\
%		$\mathcal{A}_{Rsp}(\overline{i_{Rsp}}): \mathcal{G}_{As}(\overline{o_{As}}) \land \mathcal{G}_{Ms}(\overline{o_{Ms}}) \land \mathcal{G}_{Ws}(\overline{o_{Ws}})$\\
%		$\mathcal{G}_{Rsp}(\overline{o_{Rsp}}): $ %
%		\end{tabular}}};
	
\node (gazebo) [process, below of = robotstate, yshift = -5em, xshift = -10em] {\parbox[t][][t]{3cm}{\centering Gazebo}};
%\node(gazebospec)[left of = gazebo, xshift = -12em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
%		\textbf{$\overline{i_{G}}$:} $\overline{o_{Rsp}}$\\ 
%		\textbf{$\overline{o_{G}}$:} \\
%		$\mathcal{A}_{G}(\overline{i_{G}}): \mathcal{G}_{Rsp}(\overline{o_{Rsp}})$\\
%		$\mathcal{G}_{G}(\overline{o_{G}}): $ %
%		\end{tabular}}};

\node (rviz) [process, below of = robotstate, yshift = -5em, xshift = 10em] {\parbox[t][][t]{3cm}{\centering Rviz}};
%\node(rvizspec)[right of = rviz, xshift = 8em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
%		\textbf{$\overline{i_{Rv}}$:} $\overline{o_{Rsp}}$\\ 
%		\textbf{$\overline{o_{Rv}}$:} \\
%		$\mathcal{A}_{Rv}(\overline{i_{Rv}}): \mathcal{G}_{Rsp}(\overline{o_{Rsp}})$\\
%		$\mathcal{G}_{Rv}(\overline{o_{Rv}}): $ %
%		\end{tabular}}};

\draw [arrow] (agent) to [out=-120,in= 120] node[right]{$\overline{o_A}$}(rosbridge);
\draw [arrow] (rosbridge) to [out=30,in=-30] node[right]{$\overline{o_R}$}(agent);
\draw [arrow] (rosbridge) to [out=175,in=30] node[right]{$\overline{o_R}$}(armclient);
\draw [arrow] (rosbridge) -- node[right]{$\overline{o_R}$}(mastclient);
\draw [arrow] (rosbridge) to [out=0,in=130] node[right]{$\overline{o_R}$}(wheelsclient);

\draw [arrow] (armclient) to [out=-120,in=120] node[left]{$\overline{o_{Ac}}$}(armserver);
\draw [arrow] (mastclient) to [out=-120,in= 120] node[right]{$\overline{o_{Mc}}$}(mastserver);
\draw [arrow] (wheelsclient)to [out=-120,in= 120] node[left]{$\overline{o_{Wc}}$}(wheelsserver);
\draw [arrow] (armserver) to [out=30,in=-30] node[left]{$\overline{o_{As}}$}(armclient);
\draw [arrow] (mastserver) to [out=30,in=-30] node[left]{$\overline{o_{Ms}}$}(mastclient);
\draw [arrow] (wheelsserver) to [out=30,in=-30] node[right]{$\overline{o_{Ws}}$}(wheelsclient);

\draw [arrow] (armserver) to [out=25,in=180] node[left]{}(rosbridge);
\draw [arrow] (mastserver) to [out=20,in=-10] node[right, at start, yshift =10pt, xshift =15pt ]{$\overline{o_{Ms}}$}(rosbridge);
\draw [arrow] (wheelsserver) to [out=150,in=-5] node[right]{$\overline{o_{Ws}}$}(rosbridge);

\draw [arrow] (armserver) to [out=-30,in=190] node[below]{$\overline{o_{As}}$}(robotstate);
\draw [arrow] (mastserver) -- node[right]{$\overline{o_{Ms}}$}(robotstate);
\draw [arrow] (wheelsserver) to [out=210,in=0] node[left]{$\overline{o_{Ws}}$}(robotstate);.

\draw [arrow] (robotstate) -- node[below]{$\overline{o_{Rsp}}$}(gazebo);
\draw [arrow] (robotstate) -- node[below]{$\overline{o_{Rsp}}$}(rviz);


\end{tikzpicture}}


==> dia/simplecuriosity.tex <==
\begin{figure}
\scalebox{0.8}{
\begin{tikzpicture}[node distance=6em]
\node (agent) [process] {\parbox[t][][t]{3cm}{\centering Agent}};
\node(agentspec)[above of = agent, xshift = -5em, yshift = 3em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_A}$:} $Wayp = \{A,B,C,D\}, lastvisited \in Wayp, mastready \in Bool, armready \in Bool,$\\
		\t2 $wheelsready\in Bool $ \\ 
		\textbf{$\overline{o_A}$:} $act \subseteq \{patrol(), arm(), mast()\}$\\
		$\mathcal{A}_A(\overline{i_A}):$\\
		$\mathcal{G}_A(\overline{o_A}): start \Rightarrow armready \land mastready \land wheelsready$\\
		\t2$lastvisited = A \Rightarrow act = \{patrol(B)\} \land lastvisited'=B$\\
		\t2$lastvisited = B \Rightarrow act = \{patrol(C), mast(close), arm(open)\} \land lastvisited'=C$\\
		\t2$lastvisited = C \Rightarrow act = \{patrol(D)\} \land lastvisited'=D$\\
		\t2$lastvisited = D \Rightarrow act = \{patrol(A), mast(open), arm(close)\} \land lastvisited'=A$\\
		\t2$lastvisited = origin \land start \Rightarrow act = \{patrol(A), mast(open)\} \land lastvisited'=A$\\
		\end{tabular}}};


\node (arm) [process, below of = agent, yshift = -4em, xshift = -22em] {\parbox[t][][t]{3cm}{\centering Arm}};
\node(armspec)[below of = arm, xshift = -5em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Ac}}$:} $\overline{o_R} \land \overline{o_{As}}$\\ 
		\textbf{$\overline{o_{Ac}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Ac}(\overline{i_{Ac}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{As}(\overline{o_{As}})$\\
		$\mathcal{G}_{Ac}(\overline{o_{Ac}}): g = act $ %
		\end{tabular}}};

\node (mast) [process, below of = agent, yshift = -4em] {\parbox[t][][t]{3cm}{\centering Mast}};
\node(mastspec)[below of = mast, xshift = -5em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Mc}}$:} $\overline{o_R} \land \overline{o_{Ms}}$\\ 
		\textbf{$\overline{o_{Mc}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Mc}(\overline{i_{Mc}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{Ms}(\overline{o_{Ms}})$\\
		$\mathcal{G}_{Mc}(\overline{o_{Mc}}): g = act$ %
		\end{tabular}}};


\node (wheels) [process, below of = agent, yshift = -4em, xshift = 22em] {\parbox[t][][t]{3cm}{\centering Wheels}};
\node(wheelsspec)[ below of = wheels, xshift = -5em]{\parbox[t][][t]{3cm}{\centering \begin{tabular}{l}
		\textbf{$\overline{i_{Wc}}$:} $\overline{o_R} \land \overline{o_{Ws}}$\\ 
		\textbf{$\overline{o_{Wc}}$: $Amsg = (g,f,r)$} \\
		$\mathcal{A}_{Wc}(\overline{i_{Wc}}): \mathcal{G}_R(\overline{o_R}) \land \mathcal{G}_{Ws}(\overline{o_{Ws}})$\\
		$\mathcal{G}_{Wc}(\overline{o_{Wc}}): g=act $ %
		\end{tabular}}};


\draw [arrow] (agent) to [out=175,in=30] node[right]{$\overline{o_A}$}(arm);
\draw [arrow] (agent) -- node[right]{$\overline{o_A}$}(mast);
\draw [arrow] (agent) to [out=0,in=130] node[right]{$\overline{o_A}$}(wheels);
\draw [arrow] (arm) -- node[right]{$\overline{o_{Arm}}$}(agent);
\draw [arrow] (mast) -- node[left]{$\overline{o_M}$}(agent);
\draw [arrow] (wheels) -- node[right]{$\overline{o_W}$}(agent);


\end{tikzpicture}}
\caption{Simple version of Curiosity architecture with some nodes internalised. Need to add joint config for guarantees about mast and arm. Need guarantee for wheels.}

\end{figure}
